Addressing preferred orientation in single-particle cryo-EM through AI-generated auxiliary particles

The single-particle cryo-EM field faces the persistent challenge of preferred orientation, lacking general computational solutions. We introduce cryoPROS, an AI-based approach designed to address the above issue. By generating the auxiliary particles with a conditional deep generative model, cryoPROS addresses the intrinsic bias in orientation estimation for the observed particles. We effectively employed cryoPROS in the cryo-EM single particle analysis of the hemagglutinin trimer, showing the ability to restore the near-atomic resolution structure on non-tilt data. Moreover, the enhanced version named cryoPROS-MP significantly improves the resolution of the membrane protein NaX using the no-tilted data that contains the effects of micelles. Compared to the classical approaches, cryoPROS does not need special experimental or image acquisition techniques, providing a purely computational yet effective solution for the preferred orientation problem. Finally, we conduct extensive experiments that establish the low risk of model bias and the high robustness of cryoPROS.

==> Makefile <==
all : change_tracking_v0-1_v0-2.pdf \
	  sn-article.pdf

change_tracking_v0-1_v0-2.pdf : change_tracking_v0-1_v0-2.tex
	pdflatex -interaction=nonstopmode -synctex=1 -output-directory=. $<
	bibtex change_tracking_v0-1_v0-2.aux
	pdflatex -interaction=nonstopmode -synctex=1 -output-directory=. $<
	pdflatex -interaction=nonstopmode -synctex=1 -output-directory=. $<

change_tracking_v0-1_v0-2.tex : ../v0-1/sn-article.tex sn-article.tex
	latexdiff --append-context2cmd="abstract" --graphics-markup="none" $^ > $@

sn-article.pdf : sn-article.tex
	pdflatex -interaction=nonstopmode -synctex=1 -output-directory=. $<
	bibtex sn-article.aux
	pdflatex -interaction=nonstopmode -synctex=1 -output-directory=. $<
	pdflatex -interaction=nonstopmode -synctex=1 -output-directory=. $<

clean :
	rm -f change_tracking_v0-1_v0-2.tex
	rm -f *.pdf
	rm -rf *.aux
	rm -rf *.log
	rm -rf *.bbl
	rm -rf *.blg
	rm -rf *.synctex.gz
	rm -rf *.out

